Songs Across Borders: Singable and Controllable Neural Lyric Translation

The development of general-domain neural machine translation (NMT) methods has advanced significantly in recent years, but the lack of naturalness and musical constraints in the outputs makes them unable to produce singable lyric translations. This paper bridges the singability quality gap by formalizing lyric translation into a constrained translation problem, converting theoretical guidance and practical techniques from translatology literature to prompt-driven NMT approaches, exploring better adaptation methods, and instantiating them to an English-Chinese lyric translation system. Our model achieves 99.85%, 99.00%, and 95.52% on length accuracy, rhyme accuracy, and word boundary recall. In our subjective evaluation, our model shows a 75% relative enhancement on overall quality, compared against naive fine-tuning (Code available at https://github.com/Sonata165/ControllableLyricTranslation).

==> sections/_problems.tex <==
1. Modifications compared to last meeting:
    - "Enhancing music-lyric compatibility by controlling of word boundary" seems to be proposed by a previous work "GagaST", but it does not work well. So instead of claiming "we proposed this controlling aspect", I claim "we propose a new solution to this controlling aspect", in the second point of the contribution.
    - Added "paragraph-level rhyme recommendation (Section 3.5.2)".

2. GagaST achieve word boundary control by biased decoding (re-score beam according to word boundary information). There is no direct comparison of that method and our method (it's a bit complicated to implement, and the result is foreseeable bad). Instead, the below things are used to prove our advantages:
    - We do subjective evaluation using same data as theirs, and expect we get higher "compatibility" subjective score in the testing.
    - We show the disadvantage of biased decoding on length (in Section 5.6.2 case study) and rhyme control (Sections 5.4 and 5.6.2).
    - We can mention the result they report in their paper (50~70\%, but ours is more than 90\%)

3. I put the 3 tables of Section 5.3 to the appendix because they will take too much space if put in the main body. I don't know it is acceptable to mention tables in the appendix and whether there are better solutions. (not acceptable, assume a missing appendix)


 
------------
Min - 23 Dec 9:20

Intro - 
 - Motivation
   - Needs commercial value - how many millions is lost
   - Needs strong quality gap - how bad are the translations?
   - Fig 1. 
   Should be a review of bad and good results
    - Storytelling (Inception, Leonardo D'Caprio)
    - climactic moment: related work shows weakness of others, not just a list, hint the solution
    - argument but not report
   
   Tell the readers the correct one is just what we obtained 

 - Related Work
    Is it a new task? depends on 
    
 - Method
    Make reader come up the solution from related work.


- Abstract
    shrink the motivation, add solution, and clear results with number.

- Argument
    tree-structure

==> sections/_section_length.tex <==
total:              8 p

abstract + intro:   1.5 p   1.5p
related work:       1 p     1p
method              2.5 p   2p
experiment          1 p     0.75p
result              2 p     2.5p
conclusion          0.25 p  0.25p

others:             unlimited
